Automated Synthesis of Safe Digital Controllers for Sampled-Data Stochastic Nonlinear Systems

We present a new method for the automated synthesis of digital controllers with formal safety guarantees for systems with nonlinear dynamics, noisy output measurements, and stochastic disturbances. Our method derives digital controllers such that the corresponding closed-loop system, modeled as a sampled-data stochastic control system, satisfies a safety specification with probability above a given threshold. The proposed synthesis method alternates between two steps: generation of a candidate controller pc, and verification of the candidate. pc is found by maximizing a Monte Carlo estimate of the safety probability, and by using a non-validated ODE solver for simulating the system. Such a candidate is therefore sub-optimal but can be generated very rapidly. To rule out unstable candidate controllers, we prove and utilize Lyapunov's indirect method for instability of sampled-data nonlinear systems. In the subsequent verification step, we use a validated solver based on SMT (Satisfiability Modulo Theories) to compute a numerically and statistically valid confidence interval for the safety probability of pc. If the probability so obtained is not above the threshold, we expand the search space for candidates by increasing the controller degree. We evaluate our technique on three case studies: an artificial pancreas model, a powertrain control model, and a quadruple-tank process.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios

==> discrete_pid.tex <==
% Ezio / Nicola
\section{Discrete PID Controller}
I will discuss basics for designing a digital PID controller and then we can see how to integrate this in a formal framework. In classical control theory, designing PID controllers is done in either time domain when the objectives can solely be presented in time. Alternatively, if the objectives can be translated in Laplace domain or z-domain (respectively for continuous-time and discrete-time systems), the design is preferably done in these domains.

For any continuous signal $x:\mathbb R_{\ge 0}\rightarrow\mathbb R$ we define its Laplace transform as
\begin{equation*}
X(s) = \mathcal L(x(t)) = \int_0^{\infty}x(t)e^{-st}dt.
\end{equation*}
For example Laplace transform of unit-step function $u_0(t)$ is $1/s$ and $\mathcal L(e^{at}u_0(t)) =1/(s-a)$.
For a digital signal $\{x(k),k=0,1,2,\ldots\}$ we define its z-transform as
\begin{equation*}
X(z) = \mathcal Z(x(k)) = \sum_{k=0}^{\infty}x(k)z^{-k}.
\end{equation*}
For example z-transform of unit step function $u_0(k)$ is $1/(1-z^{-1})$ and $\mathcal Z(a^k u_0(k)) = 1/(1-az^{-1})$.

All the theory of designing PID controllers is centered around linear systems.
Any linear time-invariant (LTI) system with input $u(t)$, output $y(t)$, and state $x(t)\in\mathbb R^n$, has the following dynamics
\begin{align*}
\frac{d}{dt}x(t) & = Ax(t)+ B u(t)\\
y(t) & = C x(t) + D u(t).
\end{align*}
If we bring this in Laplace domain, it becomes just a multiplication from input to output:
$Y(s) = G(s)U(s)$. The gain
$G(s) := C(sI-A)^{-1}B+D$ is called the \emph{transfer function} of the system.

A continuous PID controller in its ideal form implements the following relation:
\begin{equation*}
u(t) = K_p e(t) + K_I\int_0^t e(\tau)d\tau + K_D \frac{d}{dt}e(t).
\end{equation*}
In practice, the integral of the error also has a saturation to prevent overflow due to persistent tracking errors. This saturation is usually neglected in the design phase because of its nonlinear nature. Transfer function of a PID controller is
\begin{equation*}
C(s) = K_P + \frac{K_I}{s} + K_D s.
\end{equation*}

For designing a digital PID controller, the system is first discretized from the point of view of the controller. The digital controller with sampling time $\tau$ sees a discrete LTI system of the form
\begin{align}
x(k+1) & = G x(k)+ H u(k)\nonumber\\
y(k) & = C x(k) + D u(k),\label{eq:dis_LTI}
\end{align}
with matrices $(G,H,C,D)$ computed according to the dynamics of the continuous-time system:
\begin{equation}
\label{eq:matrices}
G(\tau) := e^{A\tau},\quad H(\tau) := \left(\int_0^\tau e^{A\lambda} d\lambda\right)B.
\end{equation}
Transfer function of LTI system \eqref{eq:dis_LTI} is $G(z) = C(zI-G)^{-1}H + D$. For the digital controller we have:
\begin{equation}
C(z) = K_P + \frac{K_I}{1-z^{-1}} + K_D(1-z^{-1}),
\end{equation}
where the \emph{trapezoidal summation} is used to approximate the integral and \emph{two-point difference} is used for the derivative term. This behavior in time domain will be the following difference equation
\begin{align}
u(k) & = u(k-1) + K_P \left[e(k)-e(k-1)\right]\nonumber\\
& + K_I e(k) + K_D[e(k)-2e(k-1)+e(k-2)].
\label{eq:PID_time}
\end{align}
Essentially, the controller needs to store the previous value of input, and previous two values of error signal.
For the closed-loop system we also have the equation
\begin{equation}
\label{eq:feedback}
e(k) = r(k)-y(k),
\end{equation}
where $r(\cdot)$ is the reference signal and $y(\cdot)$ is the output of the closed-loop system.
Figure~\ref{fig:diagram} shows the actual closed-loop diagram and its discrete version.
\begin{figure}
\includegraphics[scale=0.16]{closed_loop}
\caption{Closed-loop control: bottom diagram shows the actual continuous plant in connection with the digital controller, top diagram shows the equivalent connection from the view of controller.}
\label{fig:diagram}
\end{figure}

For a linear system, gains of a PID controller is designed according to equations \eqref{eq:dis_LTI},\eqref{eq:PID_time},\eqref{eq:feedback}
either in discrete-time or their equivalents in z domain.

Now our first challenge is that the system is nonlinear
\begin{align}
\frac{d}{dt}x(t) & = f(x(t),u(t)),\nonumber\\
y(t) & = g(x(t),u(t)).\label{eq:nonlinear}
\end{align}

My idea is to keep the nonlinear nature of the equations and discretize time, as we did for linear systems. The overall scheme is sketched in Figure~\ref{fig:scheme}.
\begin{figure}
\includegraphics[scale=0.2]{scheme}
\caption{Sketch of the synthesis approach.}
\label{fig:scheme}
\end{figure}

Consider a sampling time $T$, which might be different from sampling time of the PID controller. Then
\begin{align}
x(k+1) & = x(k) + f(x(k),u(k))T,\nonumber\\
y(k) & = g(x(k),u(k)).\label{eq:nonlinbear_disc}
\end{align}
Parameters can then be obtained based on equations \eqref{eq:nonlinbear_disc},\eqref{eq:PID_time},\eqref{eq:feedback}, which are all difference equations in discrete-time without any differential equations. The next step here would be to translate the objectives (let's say safety) into an optimization or ferasibility problem with these constraints and then solve them using nonlinear optimization or dReal, if possible.
Once we have a good guess for values for gains, we can use ProbReach to verify the closed-loop system in continuous time, that also includes differential equations.
If the spec is not verified, we can refine the first step by improving the quality of the discretization:
\begin{itemize}
\item we can take $T$ to be a fraction of actual sampling time of the controller and have a loop over equation \eqref{eq:nonlinbear_disc} to match these two.
\item we can use Taylor expansion of the dynamics to increase its quality. This requires manual differentiation of the vector field $f$.
\end{itemize}
The challenge here is to transform the required behavior to an optimization problem that can be solved efficiently over the nonlinear (discrete-time) dynamics of the system. We can discuss this in our meeting.

Another approach is to approximate the behavior of the system with a linear system around an \emph{operating point} $(x_0,u_0)$. Thus will only work if the system is not highly nonlinear.

\section{PID Synthesis in Discrete Time}
Let us denote the set of uncertain variables by $\theta$, which include the shape of meal $u_d(k)$ (time and amplitude) and measurement noise $\eta(k)$. We also group the gains of the controller in the vector $K = [K_P,K_I,K_D]$.
We formulate the following optimization
\begin{align*}
\min_K\,\,\,&\mathbb E\left[\sum_{k=0}^n e^2(k,\theta,K)\right]\\
s.t.\,\,
&x(k+1) = x(k) + f(x(k),u(k),u_d(k))T,\\
&y(k) = g(x(k)),\\
& u(k) = u(k-1) + K_P \left[e(k)-e(k-1)\right]\\
&\qquad + K_I e(k) + K_D[e(k)-2e(k-1)+e(k-2)].\\
&e(k,\theta,K) = r(k)-y(k)-\eta(k),\quad k=0,1,2,\ldots,n.
\end{align*}
In the above optimization, expectation is with respect to uncertain variables $\theta = [u_d(\cdot),\eta(\cdot)]$ and the goal is to find a set of gains that minimizes the expectation of squared error. This is a nonlinear optimization problem, which is hard to solve due to the presence of expectation operator and nonlinear functions in the constraint. In order to get an approximate sub-optimal solution for the optimization, we replace the expectation with empirical mean. In other words, we take sufficiently large samples $\{\theta^1,\ldots,\theta^N\}$ and minimize
\begin{equation*}
\min_K\,\,\,\frac{1}{N}\sum_{i=1}^N\left[\sum_{k=0}^n e^2(k,\theta^i,K)\right],
\end{equation*}
using nonlinear solvers.

Once we have a solution $K_{num}$ for this optimization, we verify it via ProbReach. If the closed-loop system violates the specification, we examine falsifying traces and their discrete counterparts. If there is a large mismatch between the two set of traces in terms of satisfying traces, we increase the quality of discretization by selecting a smaller discretization step.

\textbf{Extensions.}
\begin{itemize}
\item Using minmax optimization (worst case with respect to uncertainty) instead of minimizing expectation (average behavior).
\item using an objective function that is directly linked to falsifying specification for optimization. For instance we can use distance to the boundaries of the safe set.
\item having a smaller optimization domain first by linearizing the system and forcing the PID to make the system stable. That will put some constraints on the set of possible gains $K$.
\end{itemize}


% \paragraph{Chance-constrained formulation}
% To keep the correspondence between the ProbReach problem and its approximation, we could formulate a chance-constrained optimal control problem (CCOCP)~\cite{kouvaritakis2015stochastic}. 

% The above formulation loses connection with ProbReach as it minimizes the setpoint error (same problem if we turn it into min-max, that is typically overly conservative), while in ProbReach we want to optimize the satisfaction probability of some property. CCOCP is more adequate to this purpose as it is defined by:
% \begin{align*}
% \min_K\,\,\,&\mathbb E\left[J(K)\right]\\
% s.t.\,\,
% & \text{same as above}\\
% & \mathbf{Pr}\left[h_j(x(k)) \leq 0, \text{for all } j=1,\ldots,s  \right] \geq \beta, \quad k=0,1,2,\ldots,n.
% \end{align*}
% where $J(K)$ is the cost function for parameters $K$ (e.g., sum of squared errors), $h_j$ is a (possibly nonlinear) Borel-measurable function, $s$ is the total number of inequality constraints, and $\beta \in (0,1)$ is the lower bound for the probability that $h_j(x(k)) \leq 0$ is satisfied.

% The chance constraints better capture that we want some property (expressed as a set of inequalities) satisfies given probability bounds. 
% There are different (approximate) techniques to solve CCOCP for nonlinear systems, most of them based on sampling or linearization, see~\cite{kouvaritakis2015stochastic} for details. As explained above, sampling-based methods provide an empirical estimation of the expectation in the cost function, and for the same reason, typically support also empirical higher order moments.

% For instance, in the artificial pancreas, if we want that the probability of staying within the safe bounds (safety property) is greater than $\alpha$, we could define the following chance constraints
% $$\mathbf{Pr}\left[h_1(x(k)) \leq 0, h_2(x(k)) \leq 0 \right] \geq \sqrt[n]{\alpha}, \quad k=0,1,2,\ldots,n,$$
% where $h_1(x) = hypo - BG(x)$ and $h_2(x) = BG(x) - hyper$. 

% To maximize the probability of a reachability formula, we would need a conjunction of chance constraints of the form:
% $$\mathbf{Pr}\left[h_j(x(k)) \leq 0, \text{for all } j=1,\ldots,s  \right] \leq \beta, \quad k=0,1,2,\ldots,n,$$
% i.e., with upper probability bounds. I'm not sure this is allowed in general, but maybe is supported by sampling-based approaches.

% More complex logical formulas require the introduction of integer variables, in which I guess we are not interested.

==> qcmodel.tex <==
%%% MAIN TEXT
\subsection{Quadcopter control}
Quadcopter control is a challenging problem due to the highly non-linear dynamics connecting its rotational and translational motion. The control objective in this case is to keep the helicopter aloft. 
In~\cite{qc_model}, the author introduces a model of quadcopter dynamics and a PD control scheme able to stabilize the quadcopter in a short time ({\color{red} mention their avg stabilization time?}) after an initial perturbation of the angular velocities of the vehicle. (See Appendix \ref{app:qc_dyn} for the model equations and parameters.) Here we apply our method to synthesize controller parameters that ensure, by design, stabilization within given time bounds.

Specifically, we seek to stabilize the quadcopter in a horizontal position, which implies a zero reference signal for its roll, pitch and yaw angles, described by state variables $\phi$, $\theta$ and $\psi$ (rad), respectively. The control law for each angle monitored $a =\phi, \theta, \psi$ is:{\color{red} should we keep the integral part here?}
\begin{align*}
u_a(t) &= K_P \cdot a(t) + K_I \cdot \left( \int_{0}^{t} a(\tau) \ \mathrm{d}\tau \right) + K_D \cdot \dot{a}(t),
% u_\phi(t) &= k_p \cdot \phi(t) + k_i \cdot \left( \int_{0}^{t} \phi(\tau) \ \mathrm{d}\tau \right) + k_d \cdot \dot{\phi}(t)\\
% u_\theta(t) &= k_p \cdot \theta(t) + k_i \cdot \left( \int_{0}^{t} \theta(\tau) \ \mathrm{d}\tau \right) + k_d \cdot \dot{\theta}(t)\\
% u_\psi(t) &= k_p \cdot \psi(t) + k_i \cdot \left(\int_{0}^{t} \psi(\tau) \ \mathrm{d}\tau \right) + k_d \cdot \dot{\psi}(t),
\end{align*}
where $K_P$, $K_I$ and $K_D$ are the PID gains and the error is equal to the angle due to the zero reference signal. 

The control input $\mathbf{u}(t)$ corresponds to the angular velocities of the four rotors, $\omega_1,\ldots,\omega_4$, related to the above control laws by the following equations:
\[
\begin{bmatrix}
\omega_1^2(t)\\ \omega_2^2(t)\\ \omega_3^2(t)\\ \omega_4^2(t)
\end{bmatrix}
= \frac{T(t)}{4k} +
\begin{bmatrix}
-1 \\ -1 \\ 1 \\ 1
\end{bmatrix}
\frac{u_\phi(t)\cdot I_{xx}}{2k\cdot L} +
\begin{bmatrix}
-1 \\ 1 \\ -1 \\ 1
\end{bmatrix}
\frac{u_\psi(t)\cdot I_{zz}}{4b},
\]
where $T(t) = m\cdot g/(\cos\theta(t) \cdot \cos\phi(t))$ is the thrust, $I_{xx}$, $I_{yy}$ and $I_{zz}$ are the (constant) inertia on the $x$, $y$ and $z$ directions, $k$, $L$ and $b$ are model parameters, $m$ is the mass of the vehicle, and $g$ is the gravitational acceleration. 

The full dynamics of the system is given in Appendix~\ref{app:qc_dyn}.

{\color{red} replace with concrete values N, t1, t2, \ldots}
We wish to stabilize our quadcopter subject to time-triggered perturbations to the angles $\phi, \theta, \psi$. We define the disturbance input $\mathbf{d}(t)$ by considering $N$ perturbations at times $t_1,\ldots, t_N$. The extent of the $i$-th angle perturbation is given by uniform i.i.d. random variables $r_{\phi,i}, r_{\theta,i}, r_{\psi,i} \sim \mathcal{U}(100,200)$ deg. 

{\color{red} replace concrete values for $\tau$ and $\delta$ also here}
\paragraph{Safety property} We require that the quadcopter stabilizes within strict time bounds after each perturbation. We formulate the following invariant:
\begin{align*}
t \in [t_1 + \tau_1, t_2) &\Rightarrow (\phi \in [-\delta,\delta] \wedge \theta \in [-\delta,\delta] \wedge \psi \in [-\delta,\delta]) \wedge \\
t \in [t_2 + \tau_2, t_3) &\Rightarrow (\phi \in [-\delta,\delta] \wedge \theta \in [-\delta,\delta] \wedge \psi \in [-\delta,\delta]) \wedge \\
\ldots &\\
t \geq t_N + \tau_N &\Rightarrow (\phi \in [-\delta,\delta] \wedge \theta \in [-\delta,\delta] \wedge \psi \in [-\delta,\delta]).
\end{align*}
Note that the invariant allows for a small deviation $\delta$ around the zero angle.



%%% APPENDIX TEXT
\section{Quadcopter dynamics}\label{app:qc_dyn}
The dynamics are given by the following set of ODEs:
\begin{align*}
&\dot{\omega_x} = \tau_\phi/I_{xx} - (I_{yy} - I_{zz})\cdot \omega_y \cdot \omega_z/I_{xx}\\
&\dot{\omega_y} = \tau_\theta/I_{yy} - (I_{zz} - I_{xx})\cdot \omega_x \cdot \omega_z/I_{yy}\\
&\dot{\omega_z} = \tau_\psi/I_{zz} - (I_{xx} - I_{yy})\cdot \omega_x \cdot \omega_y/I_{zz}\\
&\begin{bmatrix}
1 & 0 & -\sin \theta \\
0 & \cos \phi & \cos \theta \sin \phi \\
0 & -\sin \phi & \cos \theta \cos \phi
\end{bmatrix}
\begin{bmatrix}
\dot{\phi} \\ \dot{\theta} \\ \dot{\psi}
\end{bmatrix}
= \omega\\
&\ddot{z} = -g + (k\cos \theta \cdot (\omega_1^2+\omega_2^2+\omega_3^2+\omega_4^2) - k_d\cdot \dot{z})/m\\
&\dot{z} = \ddot{z}
\end{align*}
where $\omega_x,\omega_y,\omega_z$ are the angular velocities of the quadcopter; $I_{xx},I_{yy},I_{zz}$ are the inertia along the $x,y,z$ directions; $\phi$, $\theta$ and $\psi$ are the roll, pitch and yaw angles, respectively; $k$ and $k_d$ are model parameters; $m$ is the mass of the vehicle; $g$ is the gravitational acceleration; $\dot{z}$ and $\ddot{z}$ are linear velocities and accelerations along the $z$ direction ($x$ and $y$ are omitted as we are not interested in modeling translation along those directions); $\omega_i$ is the angular velocity of the $i$-th rotor (see main text for its definition); $\tau_\phi$, $\tau_\theta$ and $\tau_\psi$ are the roll, pitch and yaw torques, defined by:
\begin{align*}
\tau_\phi &= L\cdot k \cdot (\omega_1^2 - \omega_3^2)\\
\tau_\theta &= L\cdot k \cdot (\omega_2^2 - \omega_4^2)\\
\tau_\psi &=  b \cdot (\omega_1^2 - \omega_2^2 + \omega_3^2 -\omega_4^2),
\end{align*}
where $L$ and $b$ are model parameters. 

Model parameters are: $L= 0.23,  k_d = 7.5 \cdot 10^{-7}, k = 5.2, m = 0.65, b = 3.13 \cdot 10^{-5}, I_{xx} = 0.0075, I_{yy} = 0.0075, I_{zz} = 0.013$.

==> stability_old.tex <==
\section{Stability Requirement}
\begin{lemma}
\label{lem:exp_bound}
Suppose $y(k+1) = \hat G y(k),\, y(0) = y_0$ with $\hat G$ having at least one eigenvalue outside the unit circle. Then there exist a constants $\beta_1>0$ and $\alpha_1>0$ and positive semi-definite matrix $\hat M_1$  such that
\begin{equation}
\label{eq:exp_linear}
\|y(k)\|^2\ge \alpha_1(1+\beta_1)^k y(0)^T \hat M_1 y(0).
\end{equation}
\end{lemma}
\begin{proof}
We cluster eigenvalues of $\hat G$ into a group of eigenvalues outside the unit circle and a group of eigenvalues on or inside the unit circle. Then there is a nonsingular matrix $T$ such that
\begin{equation*}
T \hat G T^{-1} = \left[
\begin{array}{cc}
G_1 & 0\\
0 & G_2
\end{array}
\right],
\end{equation*}
where $G_1^{-1}$ is stable. In other words, $G_1$ contains all eigenvalues of $\hat G$ from the first group.
This matrix $T$ can be found for instance by transforming $\hat G$ into its real Jordan form.
According to Lyapunov stability theory for linear systems, there are positive definite matrices $M$ and $Q$ such that the matrix equality holds
\begin{equation*}
{G_1^T}^{-1} M G_1^{-1} - M = -Q,
\end{equation*}
and we get $G_1 M G_1 - M = Q$.
Let us define
\begin{equation*}
z = Ty = \left[
\begin{array}{c}
z_1\\
z_2
\end{array}
\right] = 
\left[
\begin{array}{c}
T_1 y\\
T_2 y
\end{array}
\right],
\end{equation*}
where the partitions of $z$ and $T$ are compatible with the dimensions of $G_1$ and $G_2$. For the function $V(k) := z_1(k)^T M z_1(k)$, we have
\begin{align*}
V(k+1) - V(k) & = z_1(k+1)^T M z_1(k+1) - z_1(k)^T M z_1(k)\\
 & = z_1(k)^T (G_1^T M G_1 - M)z_1(k) = z_1(k)^T Q z_1(k)\\
 & \ge \beta_1 V(k)
\end{align*}
with $\beta_1 := \lambda_{min}(Q)/\lambda_{max}(M)$.
Then we get
$$V(k)\ge (1+\beta_1)^k V(0),\qquad \forall k\ge 1.$$
Now we write $V(k)$ in terms of $y$ as
\begin{equation*}
z_1^T M z_1 = y^T T_1^T M_1 T_1 y = y^T \hat M_1 y\le \lambda_{max}(\hat M_1)\|y\|^2,\,\,
%\end{equation*}
%\begin{equation*}
\hat M_1 := T^T \left[
\begin{array}{cc}
M & 0\\
0 & 0
\end{array}
\right] T,
\end{equation*}
%and for any initial state $y(0)$ with $T_2y(0) = 0$ we have
%\begin{equation*}
%z_1(0)^T M z_1(0) = y(0)^T \hat M_2 y(0)\ge \lambda_{min}(\hat M_2)\|y(0)\|^2,\,\,
%\hat M_2 := T^T \left[
%\begin{array}{cc}
%M & 0\\
%0 & I
%\end{array}
%\right] T.
%\end{equation*}
Then we have shown \eqref{eq:exp_linear} with
$\beta_1 := \lambda_{min}(Q)/\lambda_{max}(M)$,
$\alpha_1 = 1/\lambda_{max}(\hat M_1)$.
%and with any initial condition $y(0)$ with $T_2y(0) = 0$.
\end{proof}

Consider the following nonlinear system with additive input
\begin{equation}
\label{eq:nonl_additive}
\frac{d}{dt}x_1(t) = f(x_1(t)) + B u_1(t).
\end{equation}
Let $x_1 = 0$ be an equilibrium point for \eqref{eq:nonl_additive} and $f:D\rightarrow \mathbb R^n$ is continuously differentiable on a neighborhood of origin $D$.
Consider a digital controller with the state space representation $(G_c,H_c,C_c,D_c)$, input
$\{x_1(k\tau),\,k\in\mathbb N\}$,
and output $\{u_1(k\tau),\,k\in\mathbb N\}$,
\begin{align}
x^c_1(k+1) & = G_c x^c_1(k)+ H_c x_1(k\tau)\nonumber\\
u_1(k\tau) & = C_c x^c_1(k) + D_c x_1(k\tau).\label{eq:digital}
\end{align}
We control system \eqref{eq:nonl_additive} with digital controller \eqref{eq:digital} by setting $u_1(t) = u_1(k\tau)$ for all $t\in[k\tau,(k+1)\tau)$, $k\in\mathbb N$.

Now let us consider the same scheme but with linearized system
\begin{align}
\frac{d}{dt}x_2(t) & = A x_2(t) + B u_2(k\tau),\quad\forall t\in[k\tau,(k+1)\tau)\nonumber\\
x^c_2(k+1) & = G_c x^c_2(k)+ H_c x_2(k\tau)\nonumber\\
u_2(k\tau) & = C_c x^c_2(k) + D_c x_2(k\tau),\label{eq:linear}
\end{align}
where $A := \left.\frac{\partial f}{\partial x}(x)\right\vert_{x=0}$.
%
Define $g(x) := f(x) - A x$, thus we have
 $$\lim\limits_{\|x\|\rightarrow 0} \frac{\|g(x)\|}{\|x\|}= 0.$$
 Then for any $\gamma>0$ there exists an $r>0$ such that $\|g(x)\|\le \gamma \|x\|$ for all $x\in\mathbb R^n$ with $\|x\|\le r$.
 
Next lemma establishes an exponential bound on the difference between trajectories of the two system as long as $\|x_1(t)\|\le r$.

\begin{lemma}
\label{lem:exp_bound_diff}
Suppose both systems \eqref{eq:nonl_additive}-\eqref{eq:linear} and their controllers have the same initial state $x_1(0) = x_2(0)$ and $x_1^c(0) = x_2^c(0)$. Then the following inequality holds as long as $\|x_1(t)\|\le r$ for which $\|g(x_1(t))\|\le \gamma \|x_1(t)\|$.
\begin{equation}
\label{eq:exp_bound_diff}
\left\|\left[
\begin{array}{c}
x_1(k\tau)\\
x_1^c(k)
\end{array}
\right] - \left[
\begin{array}{c}
x_2(k\tau)\\
x_2^c(k)
\end{array}
\right] 
\right\|
\le \gamma r \alpha_2(1+\beta_2)^k.
\end{equation}
\end{lemma}
%
\begin{proof}
We first compare the two trajectories over this interval $[k\tau,k\tau+\tau)$.
\begin{align*}
& \begin{cases}
\frac{d}{dt}x_1(t) = A x_1(t) + B C_c x^c_1(k) + B D_c x_1(k\tau) + g(x_1(t))\\
x^c_1(k+1) = G_c x^c_1(k)+ H_c x_1(k\tau),
\end{cases}\\
& \begin{cases}
\frac{d}{dt}x_2(t) = A x_2(t) + B C_c x^c_2(k) + B D_c x_2(k\tau)\\
x^c_2(k+1) = G_c x^c_2(k)+ H_c x_2(k\tau)
\end{cases}\\
& \Rightarrow
\begin{cases}
\frac{d}{dt}\Delta x(t) = A \Delta x(t) + B D_c \Delta x(k\tau) + B C_c \Delta x_c(k) + g(x_1(t))\\
\Delta x_c(k+1) = G_c\Delta x_c(k) + H_c\Delta x(k\tau)\\
\end{cases}
\end{align*}
For function $W(t) = \|\Delta x(t)\|^2$, we can write
\begin{align*}
& \frac{d}{dt}W(t) = \Delta x(t)^T (A + A^T) \Delta x(t) + 2\Delta x(k\tau)^T (B D_c)^T \Delta x(t)\\
& \qquad +2 \Delta x_c(k)^T (B C_c)^T \Delta x(t) + 2 g(x_1(t)) \Delta x(t)\\
&\qquad\le \lambda_{max}(A+A^T)\|\Delta x(t)\|^2 + \|B D_c\|_2\left(\|\Delta x(t)\|^2 + \|\Delta x(k\tau)\|^2\right)\\
& \qquad + \|B C_c\|_2\left (\|\Delta x(t)\|^2 + \|\Delta x_c(k)\|^2\right) + \gamma^2 \|x_1(t)\|^2 + \|\Delta x(t)\|^2\\
& \qquad\le \theta_1 W(t) + \theta_2 W(k\tau) + \gamma^2 r^2 + \theta_3 \|\Delta x_c(k)\|^2
\end{align*}
with $\theta_2:=\|B D_c\|_2$, $\theta_3 := \|B C_c\|_2$, and 
$\theta_1 := \lambda_{max}(A+A^T)+\theta_2 +\theta_3+1$ (if $\theta_1\le 0$, we replace it with any positive quantity).
Using Gr\"{o}nwall's inequality, we get
\begin{align*}
W(k\tau+\tau)& \le e^{\theta_1\tau}W(k\tau) + \frac{e^{\theta_1\tau}-1}{\theta_1}\left[\theta_2 W(k\tau) + \gamma^2 r^2 + \theta_3\|\Delta x_c(k)\|^2\right]\\
& = (1+\gamma_1) W(k\tau) + \gamma_2\gamma^2 r^2 + \gamma_3 \|\Delta x_c(k)\|^2
\end{align*}
with properly defined positive constants $\gamma_1,\gamma_2,\gamma_3$.
We also have the following inequality for the controllers
\begin{align*}
\|\Delta x_c(k+1)\|^2& \le \|G_c\Delta x_c(k) + H_c\Delta x(k\tau)\|^2\\
& \le 2\|G_c\|_2^2 \|\Delta x_c(k)\|^2 + 2\|H_c\|_2^2 W(k\tau).
\end{align*}
Let us Define the function $F(k) := W(k\tau) + \|\Delta x_c(k)\|^2$, which satisfies the recursion
\begin{equation*}
F(k+1)\le (1+\gamma_4) F(k) + \gamma_2\gamma^2 r^2,
\end{equation*}
with $\gamma_4 := \max\left\{2\|G_c\|_2^2 + \gamma_3-1 \,,\, 2\|H_c\|_2^2 + \gamma_1\right\}.$
Initializing both systems and their controllers at the same state gives $F(0) =0$ and the exponential bound
\begin{equation*}
F(k)\le \frac{(1+\gamma_4)^k-1}{\gamma_4}\gamma_2\gamma^2 r^2,\quad k\in\mathbb N.
\end{equation*}
which gives $\sqrt{F(k)}\le \alpha_2\gamma r(1+\beta_2)^k$ with $\beta_2 = \sqrt{1+\gamma_4}-1$ and $\alpha_2 = \sqrt{\gamma_2/\gamma_4}$.
\end{proof}

\begin{theorem}
The continuous-time nonlinear system \eqref{eq:nonl_additive} controlled with the digital controller \eqref{eq:digital} is unstable 
if the linearized continuous-time system controlled by the same digital controller presented in \eqref{eq:linear} has a pole outside unit circle.
\end{theorem}

\begin{proof}
The closed-loop linearized system will have the following dynamics in discrete time
\begin{align}
x_2((k+1)\tau) & = (G+H D_c) x_2(k\tau) + H C_c x^c_2(k),\nonumber\\
x^c_2(k+1) & = G_c x^c_2(k)+ H_c x_2(k\tau),\label{eq:linear}
\end{align}
with $G = e^{A\tau}$ and $H = \int_0^\tau e^{A\lambda}Bd\lambda$.
This gives the following state transition matrix
\begin{equation}
\hat G := \left[\begin{array}{cc}
G+H D_c & H C_c\\
G_c & H_c
\end{array}
\right],
\end{equation}
which is assumed to be unstable. According to Lemma~\ref{lem:exp_bound}, there are $\beta_1>0$ and $\alpha_1>0$ and positive semi-definite matrix $\hat M_1$ such that
\begin{equation}
\label{eq:exp_linear}
\left\|\left[
\begin{array}{c}
x_2(k\tau)\\
x_2^c(k)
\end{array}
\right]\right\|^2\ge \alpha_1(1+\beta_1)^k V_0.
\end{equation}
with $V_0 := x_0^T \hat M_1 x_0$ and 
\begin{equation*}
x_0 = \left[
\begin{array}{c}
x_2(0)\\
x_2^c(0)
\end{array}
\right]
\end{equation*}
Fix an initial condition $x_0$ with $\|x_0\|=1$ and $V_0\ne 0$. Then select $n\in\mathbb N$ sufficiently large such that $\alpha_1(1+\beta_1)^n V_0>1$ and take
\begin{equation*}
0<\gamma<\frac{\sqrt{\alpha_1(1+\beta_1)^n V_0}-1}{\alpha_2(1+\beta_2)^n}.
\end{equation*}
For this $\gamma$, there exists an $r>0$ such that $\|g(x_1)\|\le \gamma\|x_1\|$ for all $x_1$ with $\|x_1\|\le r$. If trajectory of the nonlinear closed-loop system remains inside $\|x_1(t)\|\le r$ for all $t\le n\tau$, then inequality \eqref{eq:exp_bound_diff} holds and we get
\begin{equation*}
\gamma \alpha_2(1+\beta_2)^n\ge \sqrt{\alpha_1(1+\beta_1)^n V_0}-r,
\end{equation*}
due to triangular inequality for norms. This contradicts the choice of $\gamma$, thus the trajectory will visit outside of $\|x_1\|\le r$ before time $n\tau$. This proves instability of the closed-loop nonlinear system.
\end{proof}
